EgoCap: Egocentric Marker-less Motion Capture with Two Fisheye Cameras

Marker-based and marker-less optical skeletal motion-capture methods use an outside-in arrangement of cameras placed around a scene, with viewpoints converging on the center. They often create discomfort by possibly needed marker suits, and their recording volume is severely restricted and often constrained to indoor scenes with controlled backgrounds. Alternative suit-based systems use several inertial measurement units or an exoskeleton to capture motion. This makes capturing independent of a confined volume, but requires substantial, often constraining, and hard to set up body instrumentation. We therefore propose a new method for real-time, marker-less and egocentric motion capture which estimates the full-body skeleton pose from a lightweight stereo pair of fisheye cameras that are attached to a helmet or virtual reality headset. It combines the strength of a new generative pose estimation framework for fisheye views with a ConvNet-based body-part detector trained on a large new dataset. Our inside-in method captures full-body motion in general indoor and outdoor scenes, and also crowded scenes with many people in close vicinity. The captured user can freely move around, which enables reconstruction of larger-scale activities and is particularly useful in virtual reality to freely roam and interact, while seeing the fully motion-captured virtual body.

==> 4-method.tex <==
%
%
%
%
%
\section{Egocentric Inside-In Motion Capture}
\label{sec:method}

%
%
We formulate human pose estimation as inverse rendering, and use a ray-casting image formation model to optimize
%
a volumetric, actor-specific body model %
to match the captured fisheye input images.
%
This optimization is guided by one-shot joint location predictions, learned with a ConvNet-based detector and then applied to novel actors, appearance and scenes.
%
%
We combine the energy term $E_\text{color}$ for the generative model-based pose estimation with the discriminative joint location term $E_\text{detection}$ into a closed-form energy of pose $\pose$, including weak priors on pose and temporal smoothness:
%
\begin{align}
%
E(\pose) = E_\text{color}(\pose) + E_\text{detection}(\pose) + E_\text{pose}(\pose) + E_\text{smooth}(\pose)
\text{.}
\label{eqn:objective}
\end{align}

%
$E_\text{pose}(\pose_t) = 0.0001 \huber(\pose_t) + \max(\pose_t-\mathbf{l}_\text{upper})^2 + \max(\mathbf{l}_\text{lower}-\pose_t)^2$\\
$E_\text{smooth}(\pose_t) = 0.1  \huber(\pose_{t-1}+\zeta(\pose_{t-1}-\pose_{t-2})-\pose_t) $,
where $\huber$ is the smooth huberloss $\huber(x) = \epsilon \sqrt{1+\frac{x^2}{\epsilon^2}-1}$ with $\epsilon = 1$, i.e. $\huber(x) = \sqrt{1+x^2-1}$; 

%
\subsection{Volumetric Ray-Casting Model}
\label{sec:iccv-model}

\begin{figure}
	\placeholder{4cm}
	\caption{\label{fig:volumetric-model}%
		\TODO{Figure about the volumetric model}}
\end{figure}

%
%
We model the 3D body shape and pose of humans in 3D using the approach proposed by \citet{RhodiRRST2015}, which represents an actor volumetrically as a set of 91 isotropic Gaussian density functions distributed in 3D space.
%
Each Gaussian $G_q$ is parametrized by its standard deviation $\s_q$, location $\m_q$ in 3D, density $c_q$ and color~$\an_q$, which define the Gaussian shape parameters.
%
%
The combined density field of the Gaussians, $\sum_q c_q G_q$, smoothly describes the volumetric occupancy of the human in 3D space, see \cref{fig:volumetric-model}.
%
Each Gaussian is rigidly attached to one of the bones of an articulated skeleton with 16 joints \CR{the skeleton in \cref{fig:joint-transfer} (left) has more than 16 joints}, whose pose $\pose$ is parameterized with 37 %
twist pose parameters.
%
%


This representation was used in a ray-casting image formation for a general pinhole projection model.
%
A ray is cast from the camera center $\cam$ in direction $\n$ of an image pixel.
The visibility of a particular Gaussian $G_q$ along the ray ($\cam + s\n$) is computed via
%
\begin{align}
\V_q(\cam,\n,\pose) \!=\! \!\int_{0}^{\infty} \!\!\!\!\!\!\!   \exp\!\left(\!\!-\!\!\int_0^s \! \sum_i \! G_i(\cam \!+\! t \n) \dt \! \right) \! G_q(\cam \!+\! s\n) \ds
\text{.}
\label{eqn:PreciseGaussianVisibility}
\end{align}
%
This equation models light transport in a heterogeneous translucent medium \cite{Cerezo2005}, i.e. $\V_q$ is the fraction of light along the ray that is absorbed by Gaussian $G_q$.
%
The visibility is used to compute the agreement of model and observation by summing the visibility-weighted color dissimilarity $d(\cdot,\cdot)$ between image pixel $\I(u,v)$ and the Gaussian's color $\an_q$:
%
\begin{equation}
E_\text{color}(\pose,\I) = \sum_{(u,v)} \! \sum_q d(\I(u,v), \an_q) \V_q(\cam,\n(u,v),\pose) 
\text{.}
\label{eqn:ColorTermSingle}
\end{equation}
%
\citeauthor{RhodiRRST2015}'s formulation forms a good starting point for egocentric tracking, as non-stationary backgrounds and occlusions are handled well.
%
However, it applies only to static cameras, does not support the distortions of fisheye lenses, and is does not perform in real-time.

\HR{TODO: explain color distance, in supplemental?}\\
\CR{depends how complex it is}


%
\subsection{Egocentric Ray-Tracing Model}
\label{sec:ego-model}

\begin{figure}
	\placeholder{4cm}
	\caption{\label{fig:skeleton}%
		\TODO{Figure about skeleton relative to the camera rig}}
\end{figure}

In our egocentric camera rig, the cameras rigidly move with the user's head.
%
%
%
%
In contrast to commonly used skeleton configurations, where the hip is taken as the root joint, our skeleton hierarchy is rooted at the head.
%
Like a puppet, the lower body parts are then relative to the head motion, see \cref{fig:skeleton}.
%
This formulation factors out the actor's global motion, which can be estimated independently (\TODO{refer to Tango section}), and reduces the dimensionality of the pose estimation by 6 degrees of freedom.
The movable camera is reduced to a static camera formulation such that \cref{eqn:PreciseGaussianVisibility} still applies \CR{why should that be a problem?}, including its analytic derivatives which are crucial for efficient optimization.

%
Simply undistorting the fisheye images before optimization is impractical as resolution at the image center reduces and pinhole cameras cannot capture fields of view approaching 180 degrees for their image planes would need to be infinitely large.
%
To apply ray-casting formulation described in the previous section to our egocentric motion-capture rig, with its 180\textdegree field of view, we replace the original pinhole camera model with the omnidirectional camera model of \citet{ScaraMS2006}.
%
The ray direction $\n(u,v)$ of a pixel $(u,v)$ is then given by
$\n(u,v) \!=\! [u, v, f(\rho)]^{\!\top}$, where $f$ is a polynomial of the distance $\rho$ of $(u, v)$ to the estimated image center.
%
%
%
%
%
%
%
%
%
%
%
We combine the model-based energy terms (\cref{eqn:ColorTermSingle}) for the two cameras in our egocentric camera rig using
%
\begin{align}
E_\text{color}(\pose) = \lambda_\text{color} \cdot \left(
	E_\text{color}(\pose, \I_\text{left}) + 
	E_\text{color}(\pose, \I_\text{right})
\right) \text{.}
\label{eqn:ColorTerm}
\end{align}

%


%
\section{Egocentric Joint Location Detection}
\label{sec:detections}

In our approach, we combine the generative, model-based motion capture method described in the previous section with a discriminative joint location detector learned from annotated egocentric fisheye images.
%
By incorporating joint detections into our egocentric motion capture approach, we dramatically improve the quality of reconstructed poses, make them more robust to tracking failures and enable efficient recovery after tracking failures.
%
Recent advances in the design and training of deep convolutional networks (ConvNets) led to standard network architectures that are applicable to a wide variety of computer vision applications \citep[e.g.][]{KrizhSH2012,SimonZ2015}.
%
To apply these architectures to a new application domain, such as egocentric fisheye video in our case, the largest burden is to gather and annotate training datasets that are sufficiently large and varied, containing tens of thousands of images with a variety of human activities.


We use the body-part detector of \citet{InsafPAAS2016}, which is showing state-of-the-art results on human pose estimation from single images.
%
This network was trained on the MPII Human Pose dataset \citep{AndriPGS2014}, which contains \texttildelow 19,000 internet images that were manually annotated in a crowd-sourced effort, combined with the Leeds Sports Extended dataset \citep{JohnsonCVPR2011} of 10,000 images.
%
However, the network does not generalize to the top-down perspective and fisheye distortion of our novel egocentric camera setup;
%
we therefore create a new training dataset that is tailored for our egocentric motion capture setup.
%
%
%
As our camera rig is novel, there are no existing public datasets we can use, and we thus create our own dataset from scratch. %


%
%
\subsection{Dataset Creation}
\label{sec:dataset}

\begin{figure}
%
%
	\includegraphics[width=\linewidth]{figures/joint-transfer-v2}%
	\caption{\label{fig:joint-transfer}%
		The skeleton estimated from the multi-view motion capture system (left), is converted from global coordinates (center) into each fisheye camera's coordinate system (right) via the checkerboard.}
\end{figure}

We propose a novel approach for semi-automatically creating large, realistic training datasets for human pose estimation that comprise tens of thousands of camera images annotated with the joint positions of a kinematic skeleton.
%
To avoid the tedious and error-prone manual annotation of the joint locations in thousands of images, as in previous work, we use a state-of-the-art markerless motion capture system \CR{cite Captury Studio or \citet{StollHGST2011}?} to estimate the joint locations in 3D from eight stationary cameras, and then project them into the fisheye images of our head-mounted camera rig.
%
This requires tracking the rigid motion of our head-mounted camera rig relative to the stationary cameras of the motion capture system, for which we use a large checkerboard rigidly attached to our camera rig (\cref{fig:joint-transfer}).
%
We detect this checkerboard in all stationary cameras in which it is visible, and triangulate the 3D positions of its corners to estimate the pose and orientation of the camera rig.
%
Using \citeauthor{ScaraMS2006}'s camera distortion model, we then project the 3D joint locations into the fisheye images recorded by our camera rig.

%


%
\paragraph{Dataset Augmentation}
%
%
We record video sequences of multiple actors performing various motions in a green-screen studio, so that we can replace the background using chroma keying.
%
%
We replace the background of each video frame with a random, floor-related image from Flickr, as our fisheye cameras mostly see the ground below the tracked actor.
%
In addition, we augment the the appearance of actors by varying the colors of clothing, while preserving shading effects, using intrinsic recoloring \cite{MekaZRT2016}.
%
This is, to our knowledge, the first application of intrinsic recoloring for augmenting datasets.
%
We furthermore exploit the shared plane of symmetry of our camera rig and the human body to train a single detector on a dataset twice the size by mirroring the images and joint location annotations of the right-hand camera to match those of the left-hand camera during training, and vice versa during motion capture.
%
We also apply a random gamma curve ($\gamma \!\in\! [\text{0.5}, \text{2}]$) to simulate changing lighting conditions, and during training of detectors randomly scale images by up to $\pm$15 in size to be more robust to variations in actor size.
%
As we will demonstrate, this data augmentation process results in a learned joint detector that is robust to a large variety of backgrounds, changing illumination and clothing colors, %
even though the training dataset is only based on recordings of people with six different sets of clothing.
%
Our complete training dataset is created from recordings of six actors totaling \texttildelow 21 minutes at 30\,Hz.
%
Thanks to our randomized augmentation, we can use every single video frame in our training dataset despite the very similar poses in consecutive video frames, as both background and clothing colors are different for every frame (see \cref{fig:augmentation}).
%
This results in a dataset of \texttildelow 75,000 fisheye images with annotated joint locations.


\begin{figure}
	\inputTikZfigure{augmentation}\vspace{-0.5em}%
	\caption{\label{fig:augmentation}%
		Illustration of our dataset augmentation using randomized backgrounds, intrinsic recoloring and gamma jittering.
		Note the varied shirt colors as well as brightness of the trousers and skin, which help prevent overtraining of the ConvNet-based joint detector.}
\end{figure}


%
\subsection{Detector Learning}
\label{sec:learning}

We begin with the 101-layer ConvNet \citep{HeZRS2015} trained by \citet{InsafPAAS2016} for 2D pose estimation.
We remove the original prediction layers and replace them with the ones that output 18 body part heatmaps.
Input frames are rescaled to 640$\times$512 size, such that the average diameter of a human body is \texttildelow 320\,px.
The predicted heatmaps are of 8$\times$ coarser resolution.
We then finetune the networks to our dataset for 3 epochs with the learning rate 0.002, and drop it to 0.0002 for 4 additional epochs.
Parameters of \TODO{…}

\TODO{Eldar: evaluation of detectors}


%
\subsection{Joint-Detection Energy}
\label{sec:detections-energy}
%
%
%
%
%
%

The learned detections, in the form of heatmaps (see \cref{fig:heatmapsOutput}), are integrated in the objective energy as a soft constraint.
%
For each detection label, a special 3D Gaussian is attached to the corresponding skeleton joint, and the agreement of the Gaussian's position and the joint location prediction is computed by replacing $d(\cdot,\cdot)$ in \cref{eqn:ColorTermSingle} with the detection confidence at pixel $(u,v)$.
%
$E_\text{detection}$ is then defined as the sum over the detection agreements of all labels, for both cameras, and weighted by $\lambda_\text{detection}$.
%
A similar approach was introduced by \citet{ElhayAJTPABST2015}, and later generalized to the volumetric density model we use by \citet{HelgeECCVSubmission}.


\begin{figure}
	\inputTikZfigure{detection}\vspace{-0.5em}%
	\caption{\label{fig:heatmapsOutput}%
		Color coded joint position detection.
		For crowded scenes (left), detections can be multi modal (center), however the maximum (right) is dominantly on the user. Knee, hand, and foot locations are here excluded for clarity of exposition.}
\end{figure}

%
\subsection{Real-Time Optimization}
\label{sec:optimization}

\citeauthor{RhodiRRST2015}'s volumetric ray-casting method models occlusion as a smooth phenomenon by integrating the visibility computations within the objective function instead of applying a depth test once before optimization.
%
While this is beneficial for optimizing disocclusions, it introduces dense pairwise dependencies between all Gaussians:
%
the visibility $\V_q$ (\cref{eqn:PreciseGaussianVisibility}) can be evaluated in linear time in terms of the number of Gaussians, $N_q$, but computing its gradient with respect to the position of all Gaussians, which is required for gradient-based optimization, has quadratic complexity in $N_q$. %


To nevertheless reach real-time performance, we introduce a new parallel stochastic optimization approach.
%
The ray-casting formulation allows a natural parallelization of $E_\text{detection}$ and $E_\text{color}$ (\ref{eqn:ColorTerm}) \CR{what about other energy terms?}\HR{OK?}\CR{I mean $E_\text{pose}$ and $E_\text{smooth}$} and its gradient computation across pixels $(u, v)$ and Gaussians $G_q$.
%
We also introduce a traversal step, which determines the Gaussians which are in the proximity for each ray, and excludes distant Gaussians with negligible contribution to the energy.
%
These optimizations lead to significant run-time improvements, particularly when executed on a GPU,
%
but only enable interactive frame rates.


We achieve further reductions in run times by introducing a statistical optimization approach that is tailored to the ray-casting framework.
%
The input image pixels are statistically sampled for each gradient iteration step, as proposed by \citet{BlanzV1999}.
%
In addition, we sample the volumetric body model by excluding Gaussians from the optimization at random.
\TODO{Bla Bla}
Due to the quadratic dependency on the number of Gaussians, execution time is significantly reduced to real-time frame rates of \TODO{} fps.


\paragraph*{Initialization by ECCV paper}
Silhouette fitting?

